Scalar-Scaffolded Gluons and the Combinatorial Origins of Yang-Mills Theory

We present a new formulation for Yang-Mills scattering amplitudes in any number of dimensions and at any loop order, based on the same combinatorial and binary-geometric ideas in kinematic space recently used to give an all-order description of Tr $\phi^3$ theory. We propose that in a precise sense the amplitudes for a suitably "stringy" form of these two theories are identical, up to a simple shift of kinematic variables. This connection is made possible by describing the amplitudes for $n$ gluons via a "scalar scaffolding", arising from the scattering of $2n$ colored scalars coming in $n$ distinct pairs of flavors fusing to produce the gluons. Fundamental properties of the "$u$-variables", describing the "binary geometry" for surfaces appearing in the topological expansion, magically guarantee that the kinematically shifted Tr $\phi^3$ amplitudes satisfy the physical properties needed to be interpreted as scaffolded gluons. These include multilinearity, gauge invariance, and factorization on tree- and loop- level gluon cuts. Our "stringy" scaffolded gluon amplitudes coincide with amplitudes in the bosonic string for extra-dimensional gluon polarizations at tree-level, but differ (and are simpler) at loop-level. We provide many checks on our proposal, including matching non-trivial leading singularities through two loops. The simple counting problem underlying the $u$ variables autonomously "knows" about everything needed to convert colored scalar to gluon amplitudes, exposing a striking "discovery" of Yang-Mills amplitudes from elementary combinatorial ideas in kinematic space.

==> Sections/7_LoopCut.tex <==
\section{Integrand Cuts: Tree-loop cut and loop-cut}
\label{sec:Loopcut}

We finally turn to the most non-trivial checks on our proposal. We will consider the residues of our curve integral at loop level, on a ``single cut'' setting a single loop propagator to zero. By consistency, this should match the ``forward limit'' of an amplitude with one loop lower.
Now this match is usually fraught with subtlety in non-supersymmetric theories, due to the fact that both single-cuts and forward limits are naively infected with ``1/0" divergences. But as we have already mentioned, the labelling of variables on surfaces gives us a way out of this impasse, at least allowing a non-trivial comparison between ``loop cut'' and ``forward limit'' to be made.

In this section, we will focus on showing this connection at one loop. We will see that if we cut any loop propagator at one loop, it matches the tree-level amplitude in the forward limit, with the cut loop adding two color-adjacent particles,  ``glued'' by summing over polarization states. This will hold not only in the field theory limit but even at finite $\alpha^\prime$. 

We will do this by examining the single-cut and forward-limit integrands. We will see that due to a number of new properties of $u$ variables we first encounter here--hardwired into their combinatorial definition--the two integrands beautifully match, up to a total derivative in the $y$ variables. 

While our proof of ``loop-cut = forward limit'' in this section is strictly valid at one loop, as we will see the character of the argument is quite ``local" to the loop being cut, and one can expect the argument to be extendable to general surfaces.

Note also that correctly matching the single loop cut, together with our earlier proof of the correct ``tree-like'' factorization, automatically implies that all the leading singularities computed in the previous section must be correctly matched at one loop. An extension of the loop cut argument to all loop orders would similarly guarantee inter-alia the matching of all leading singularities, and the non-trivial matching of two-loop leading singularities in the previous section bolsters the belief that the loop-cut matching should work at all loops.  

\subsection{Set up}
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/Loop_cut2.png}
\caption{Tadpole Triangulation with $Y_{1}$ and $X_{1,1,}$ and loop cut.}
\label{fig:LoopCut}
\end{center}
\end{figure}
On the loop side, we will be considering a $2n$-scalar 1-loop amplitude, from which we get the $n$-point 1-loop gluon amplitude. To define the corresponding surface, we will find it convenient to pick a particular ``tadpole'' triangulation, whose fat-graph includes the loop propagator $Y_1$ as well as the tadpole propagator $X_{1,1}$ (see figure \ref{fig:LoopCut}). Taking the loop cut corresponds to extracting the residue when $Y_1=0$, which is easy to do in this triangulation since $Y_1$ is one of the chords in the triangulation. The resulting tree-level result corresponds to a $(2n+2)$-point amplitude, with the two extra gluon legs glued. We call these extra two legs $1^\prime$ and $p$ (see figure \ref{fig:LoopCut}). 
Regardless of $Y_1=0$ we still keep $X_{1,1}$ as the label of the curve on the cut surface. 

To do the matching, we consider the tree-level amplitude of $2n+4$ scalars, where we label the particles as $(1,2,...,2n,1^\prime,s_R,p,s_L)$ so that the matching with the loop computation becomes clearer.
We make the gluons, $1^\prime$ and $p$, on-shell by taking the scaffolding residue, $X_{1,p}=X_{1^\prime,p}=0$. Therefore we pick a triangulation to define the surface that contains propagators $\{X_{1,p},X_{1,p^\prime},X_{1,1^\prime}\}$, the last propagator is chosen to replicate the triangulation picked in the loop cut part (see figure \ref{fig:TreeGlue}). 
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/TreeGlue.png}
\caption{Tree triangulation and scaffolding residue.}
\label{fig:TreeGlue}
\end{center}
\end{figure}
The corresponding fat graphs associated with the 1-loop and tree-level triangulations are presented in figure \ref{fig:FatGraphs}. 

\subsection{Gluing in Momentum Space}

We will now describe the procedure for performing the polarization sum (``gluing'') for the two gluons in the forward limit opened up by cutting a loop. This will be a bit more interesting than the gluing we already encountered in our discussion of tree-level factorization, where we took two separate gauge-invariant objects ${\cal A}_L^\mu(p, \cdots), {\cal A}_R^\nu(-p,\cdots)$ and performed the polarization sum over the intermediate particle which finally yielded (thanks to the gauge-invariance of ${\cal A}_L,{\cal A}_R$) the trivial gluing rule ${\cal A}_L^\mu {\cal A}_R^\nu \eta_{\mu\nu}$. Now instead here we wish to start with a single $n$-point tree-level amplitude, and glue together two of its adjacent legs, say $1$ and $n$. The polarization sum is:
\begin{equation}
	{\cal A}_{\text{glued}}= {\cal A}_n^{\mu \nu} \left( -\eta_{\mu,\nu} + \frac{p_\mu q_\nu + p_\nu q_\mu}{p \cdot q} \right), \quad \text{with} \quad {\cal A}_n^{\mu \nu}= \partial_{\epsilon_{1,\mu}} \partial_{\epsilon_{n,\nu}} {\cal A}_n.
\end{equation} 

Now, there is a crucial difference with the tree-like gluing case. Gauge invariance does {\bf not} imply that ${\cal A}_n^{\mu \nu} p_\mu$ vanishes, and in general for non-Abelian gauge theories we have 
\begin{equation}
	{\cal A}_n^{\mu \nu}p_{\mu} \neq 0.
\end{equation}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\textwidth]{Figures/FatGraphs2.png}
\caption{1-loop fat graph (left) and tree-level fat graph (right).}
\label{fig:FatGraphs}
\end{center}
\end{figure}

This is famously related to the need to introduce ghost fields in the Lagrangian at loop level. However all is not lost, gauge invariance still constrains the form of this object, since we must have:
\begin{equation}
	{\cal A}_n^{\mu \nu}p_{\mu} p_{\nu} = 0 \quad \Rightarrow \quad {\cal A}_n^{\mu \nu}p_{\mu} = \mathcal{N} \, p^{\nu},
\end{equation}
where $\mathcal{N}$ is some function of the remaining kinematics and polarizations. Using this fact, the result after gluing can be written as:
\begin{equation}
	{\cal A}_{\text{glued}} = {\cal A}_n^{\mu \nu} \left( -\eta_{\mu,\nu} + \frac{p_\mu q_\nu + p_\nu q_\mu}{p \cdot q} \right)=- {\cal A}_n^{\mu \nu}\eta_{\mu,\nu} + 2 \mathcal{N},
\end{equation}
where the $q^{\mu}$ dependence dropped out again, as expected. Therefore, to perform the gluing in the forward limit, we need to determine $\mathcal{N}$. 

Let us now rephrase some of these statements in scalar language using the $X_{i,j}$'s from the scaffolded gluon amplitude. Again, let us say we start with an $n$-point tree-level gluon amplitude, so $2n$ scalar amplitude, and we want to glue gluons $1$ and $n$. Then the $X$'s associated with the polarizations of these gluons are, respectively, $X_{2}^{\mu}$ and $X_{2n}^{\nu}$, so we have:
\begin{equation}
	{\cal A}_n^{\mu \nu} = \frac{\partial^2{\cal A}_n}{\partial X_2^\mu \partial X_{2n}^\nu},
\end{equation}
where ${\cal A}_n$ stands for the amplitude obtained after taking the scaffolding residue in gluons $1$ and $n$. Now, gauge invariance and multi-linearity in particles $1$ and $n$, we know we can write:
\begin{equation}
	{\cal A}_n = \sum_j (X_{2,j} - X_{1,j}) \mathcal{Q}^2_j = \sum_j (X_{2n,j} - X_{1,j}) \mathcal{Q}^{2n}_j.
	\label{eq:glueginv}
\end{equation}

Now by linearity in the polarizations the $\mathcal{Q}^2_j$ cannot depend in $X_{2,k}$ for any $k$, and similarly for $\mathcal{Q}^{2n}_j$. Therefore we can rewrite \eqref{eq:glueginv} as:
\begin{equation}
	{\cal A}_n = \sum_j (X_{2,j} - X_{1,j}) \frac{\partial {\cal A}_n}{\partial X_{2,j}} = \sum_j (X_{2n,j} - X_{1,j}) \frac{\partial {\cal A}_n}{\partial X_{2n,j}}.
\end{equation}

Now plugging the second form of ${\cal A}_n$ into the derivative with respect to $X_{2,j}$, we get:
\begin{equation}
	{\cal A}_n = \sum_{j,k} (X_{2,j} - X_{1,j})(X_{2n,k} - X_{1,k})  \frac{\partial^2 {\cal A}_n}{\partial X_{2,j}\partial X_{2n,k}} + X_{2,2n} \frac{\partial {\cal A}_n}{\partial X_{2,2n}}.
\end{equation}
From this expression we can read off ${\cal A}_n^{\mu \nu}$:

\begin{equation}
	{\cal A}_n^{\mu \nu} = 4 \sum_{j,k} (X_2^\mu - X_j^\mu) (X_{2n}^\nu - X_{k}^\nu) \frac{\partial^2 {\cal A}_n}{\partial X_{2,j}\partial X_{2n,k}} -2 \eta^{\mu\nu} \frac{\partial {\cal A}_n}{\partial X_{2,2n}}.
\end{equation}
Now doing a gauge transformation and a rescaling in gluon $2$ and $2n$, let us choose $X_2^\mu = X_1^\mu$ and $X_{2n}^\nu = X_1^\nu$. So we get the following representation of ${\cal A}_n^{\mu \nu}$:

\begin{equation}
	{\cal A}_n^{\mu \nu} \propto 4 \sum_{j,k} (X_1^\mu - X_j^\mu) (X_{1}^\nu - X_{k}^\nu) \frac{\partial^2 {\cal A}_n}{\partial X_{2,j}\partial X_{2n,k}} - 2\eta^{\mu\nu} \frac{\partial {\cal A}_n}{\partial X_{2,2n}}.
\end{equation}
Now this is a particularly nice representation because it is such that $\mathcal{N}$ is zero:
\begin{equation}
\begin{aligned}
	{\cal A}_n^{\mu \nu}p_{\mu} &\propto \left[4 \sum_{j,k} (X_1^\mu - X_j^\mu) (X_{1}^\nu - X_{k}^\nu) \frac{\partial^2 {\cal A}_n}{\partial X_{2,j}\partial X_{2n,k}} -2 \eta^{\mu\nu} \frac{\partial {\cal A}_n}{\partial X_{2,2n}}\right] (X_3-X_1)_{\mu} \\
	&= 2 \sum_{j,k} (X_{3,j} - X_{1,j}) (X_{1}^\nu - X_{k}^\nu) \frac{\partial^2 {\cal A}_n}{\partial X_{2,j}\partial X_{2n,k}} -2 (X_3^\nu-X_1^\nu) \frac{\partial {\cal A}_n}{\partial X_{2,2n}} \\
	& = 2\sum_k (X_{1}^\nu - X_{k}^\nu) \frac{\partial }{\partial X_{2n,k}} \underbrace{\left( \sum_j (X_{3,j} - X_{1,j})\frac{\partial {\cal A}_n}{\partial X_{2,j}} \right)}_{=0} - 2 (X_1^\nu - X_3^\nu)\frac{\partial {\cal A}_n}{\partial X_{2,2n}} \\
	& \quad \quad +2 (X_1^\nu-X_3^\nu) \frac{\partial {\cal A}_n}{\partial X_{2,2n}} \\
	&=0,
\end{aligned}
\end{equation}
where the sum over $j$ vanishes because of gauge invariance. Therefore we found a representation of ${\cal A}_n^{\mu \nu}$ for which $\mathcal{N}=0$, and so in which the gluing becomes simply:
\begin{equation}
\begin{aligned}
	{\cal A}_{\text{glued}} &\propto -{\cal A}_n ^{\mu \nu} \eta_{\mu \nu} \propto 2 \sum_{j,k} (X_1^\mu -X_j^\mu)(X_{1\mu} - X_{k\mu}) \frac{\partial^2 {\cal A}_n}{\partial X_{2,j}\partial X_{2n,k}} -D \frac{\partial {\cal A}_n}{\partial X_{2,2n}} \\
	&=  \sum_{j,k} (X_{1,j} + X_{1,k} - X_{j,k})  \frac{\partial^2 {\cal A}_n}{\partial X_{2,j}\partial X_{2n,k}} -D \frac{\partial {\cal A}_n}{\partial X_{2,2n}} .
\end{aligned}
\label{eq:glue}
\end{equation}

This is finally our expression for gluing in the forward limit, written purely in terms of $X$ variables. 

Of course, this holds for gluing any gauge-invariant object in the forward limit, but we now turn to the specific representations we give for $M$ in terms of integrals of forms of $y$ variables, and translate this statement into a gluing rule for these forms. Let's start by defining the two forms we obtain by taking one scaffolding residue after the other:
\begin{equation}
    \Omega_{s_{1,3}} = \text{Res}_{y_{1,3}=0} \Omega_{2n}^{\text{loop}}, \quad \Omega_S = \text{Res}_{y_{1,2n-1}=0} \Omega_{s_{1,3}}.
\end{equation}

Then we have:
\begin{equation}
\begin{aligned}
	\frac{\partial {\cal A}_n}{\partial X_{2,j}} &= \int \frac{\partial \Omega_S}{\partial X_{2,j}} = \int\text{Res}_{y_{1,2n-1}=0} \left( \frac{\partial \Omega_{s_{1,3}}}{\partial X_{2,j}} \right) \\
 &=\int\text{Res}_{y_{1,2n-1}=0} \left(\prod_{s\neq (1,3)} \frac{\diff y_{s}}{y_{s}^2} \, \prod_{i} \frac{\diff y_{i}}{y_{i}^2} \times \frac{\partial \log ( u_{2,j})}{\partial y_{1,3}}\prod_{(k,m) \neq \{(1,j),(2,j)\}} u_{k,m}^{ X_{k,m}}[y] \bigg \vert_{y_{1,3}=0}\right) \\ 
 &=  \int\prod_{\substack{s\neq \{(1,3),\\(1,2n-1)\}}} \frac{\diff y_{s}}{y_{s}^2} \, \prod_{i} \frac{\diff y_{i}}{y_{i}^2}  \left[ \sum_{k} 	(X_{2n,k}-X_{2n-1,k})\frac{\partial \log ( u_{2,j})}{\partial y_{1,3}}  \frac{\partial \log ( u_{2n,k})}{\partial y_{1,2n-1}} \right.\\
 & \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad  \quad \quad \left. + \frac{\partial^2 \log ( u_{2,2n})}{\partial y_{1,3} \partial y_{1,2n-1}}   \right]\times \prod_{\substack{(k,m) \neq \{(1,j),(2,j),\\
 (1,k),(2n-1,k)\}}} u_{k,m}^{ X_{k,m}}[y] \bigg \vert_{y_{1,3}=y_{1,2n-1}=0},
\end{aligned}
\end{equation}
which further taking a derivative on $X_{2n,k}$, gives
\begin{equation}
\begin{aligned}
	\frac{\partial^2 {\cal A}_n}{\partial X_{2n,k}\partial X_{2,j}} =  \int &\underbrace{\prod_{\substack{s\neq \{(1,3),\\(1,2n-1)\}}} \frac{\diff y_{s}}{y_{s}^2} \, \prod_{i} \frac{\diff y_{i}}{y_{i}^2}  \prod_{\substack{(k,m) \neq \{(1,j),(2,j),\\
 (1,k),(2n-1,k)\}}} u_{k,m}^{ X_{k,m}}[y]   }_{\tilde{\text{(KN)}}}\\
 &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left(\frac{\partial \log ( u_{2,j})}{\partial y_{1,3}}  \frac{\partial \log ( u_{2n,k})}{\partial y_{1,2n-1}} \right) \bigg \vert_{y_{1,3}=y_{1,2n-1}=0} , 
\end{aligned}
\end{equation}
so we can summarize the gluing rule as follows:
\begin{equation}
	\mathcal{A}_{\text{Glued}} =\int \sum_{j,k}\left(X_{1,j}+X_{1,k}-X_{j,k} \right) \frac{\partial \log{(u_{2,j})}}{\partial y_{1,3}} \frac{\partial \log (u_{2n,k})}{\partial y_{1,2n-1}} \times \tilde{\text{(KN)}} -D \, \cdot \frac{\partial \Omega_S }{\partial X_{2,2n}}.
	\label{eq:glue2}
\end{equation}

We finally translate this result using the variables of the loop-cut we want to compute, and find that the glued form is given by: 
\begin{equation}
\begin{aligned}
	\Omega^{2n}_{\text{Glued}} =& \prod_i \frac{\diff y_i}{y_i^2} \prod u_C^{X_C} \left.\left[\sum_{\substack{j\in\{2,\dots,1^\prime \}, \\ \,k \in \{1,\dots,2n\}} }\left(X_{p,j}+X_{p,k}-X_{j,k} \right) \frac{\partial \log{u_{s_L,j}}}{\partial y_{1,p}} \frac{\partial \log u_{s_R,k}}{\partial y_{1^\prime,p}} \right] \right\vert_{y_{1,p}=y_{1^\prime,p}=0} \\
 & \,-D \, \cdot \frac{\partial \Omega_S}{\partial X_{s_L,s_R}}  ,  
\end{aligned}
\end{equation}
where $y_i$ are now all remaining variables in the triangulation (other than the two scaffolding ones we extracted the residue) and $C$ stands for the curves living in the smaller surface, obtained after taking the scaffolding residue. $\Omega_S$ is now the form resulting from taking both scaffolding residues that now correspond to $y_{1,p}=y_{1^\prime,p}=0$.
  
Now it is particularly useful to reorganize this equation in the following way:
\begin{equation}
\begin{aligned}
\Omega^{2n}_{\text{Glued}} =& - \underbrace{ D \, \cdot \frac{\partial \Omega_S}{\partial X_{s_L,s_R}}}_{(\dagger)} \quad + \quad  \prod_i \frac{\diff y_i}{y_i^2} \prod u_C^{X_C} \left[ - \underbrace{\sum_{j,k\in\{2,\dots,2n \}} X_{j,k} \frac{\partial \log{u_{s_L,j}}}{\partial y_{1,p}} \frac{\partial \log u_{s_R,k}}{\partial y_{1^\prime,p}}}_{(\dagger \dagger)} \right. \\
	&  + \underbrace{\sum_{j\in\{2,\dots,2n \}} X_{p,j} \left( \frac{\partial \log{u_{s_L,j}}}{\partial y_{1,p}} \sum_{k \in \{1,\dots,2n\}} \frac{\partial \log u_{s_R,k}}{\partial y_{1^\prime,p}} + \frac{\partial \log u_{s_R,j}}{\partial y_{1^\prime,p}} \sum_{k \in \{2,\dots,1^\prime\}} \frac{\partial \log u_{s_L,k}}{\partial y_{1,p}} \right)}_{(\dagger \dagger \dagger)}  \\
	&  - \underbrace{\sum_{k \in \{2,\dots,2n\}}X_{1^\prime,k} \left( \frac{\partial \log{u_{s_L,1^\prime}}}{\partial y_{1,p}}  \frac{\partial \log u_{s_R,k}}{\partial y_{1^\prime,p}} \,+ \frac{\partial \log{u_{s_L,k}}}{\partial y_{1,p}}  \frac{\partial \log u_{s_R,1}}{\partial y_{1^\prime,p}} \right)}_{(\dagger \dagger \dagger \dagger)}\\
	& \left. \left. \underbrace{-X_{1,1^\prime} \left( \frac{\partial \log{u_{s_L,1^\prime}}}{\partial y_{1,p}}  \frac{\partial \log u_{s_R,1}}{\partial y_{1^\prime,p}}  \right)}_{(\dagger \dagger \dagger \dagger \dagger)} \right] \right\vert _{y_{1,p}=y_{1^\prime,p}=0},
\end{aligned}
\end{equation}
where we are setting $X_{1,j}=X_{1\prime,j}$.
Our goal now is to show the different terms agree with the loop cut result, up to a possible total derivative. Let's look at what the loop-cut result looks like before proceeding. 
\subsection{Loop-cut }
As explained before, in the loop integrand we include all the curves up to self-intersection one. So by taking the residue on $Y_1$, we are effectively taking the residue of the integrand at $y_1=0$, which leads to:
\begin{equation}
\begin{aligned}
	\text{Res}_{y_1=0} \Omega_{2n}^{\text{loop}} =&  \prod_i \frac{\diff y_i}{y_i^2} \prod u_C^{X_C} \left[ \sum_{j \in \{2,\dots,2n\}} Y_j \frac{\partial \log{u_{Y_j}}}{\partial y_{1}} + \sum_{j<k \in \{2,\dots,2n\}} X_{k,j}  \frac{\partial \log{u_{k,j}}}{\partial y_{1}} \right. \\
	& \left. \left. + X_{1,1} \frac{\partial \log{u_{1,1}}}{\partial y_{1}} \quad + \sum_{k \in \{2,\dots,2n\}}  X_{k,k} \frac{\partial \log{u_{k,k}}}{\partial y_{1}} \quad  - \Delta \right] \right\vert _{y_{1,p}=y_{1^\prime,p}=0}.
\end{aligned}
\label{eq:loopcut1}
\end{equation}

\textcolor{red}{Copied from letter.}
\begin{equation}
    \mathop{\mathrm{Res}}_{X_{a,p}=0}\left(\Omega_{2n}^{\text{loop}}\right) = \sum_{j,k} \left[\left(X_{j,p} + X_{k,p} - X_{k,j} \right)\frac{\partial^2 \mathcal{A}_{n+2}^\mathcal{S}}{\partial X_{j,x}\partial X_{k,x^\prime}} \right]\bigg\vert_{a^\prime\rightarrow a} -D \frac{\partial \mathcal{A}_{n+2}^{\mathcal{S}}}{\partial X_{x^\prime,x}}; \quad j,k \in (a,a+1,\cdots,a-1, a^\prime).
    \label{eq:loop-cut}
\end{equation}

For the matching, we set $ X_{k,k}=0$ for all $k\neq1$. So, using $\Delta = 1-D$, we can rewrite \eqref{eq:loopcut1} as follows:
\begin{equation}
\begin{aligned}
	\text{Res}_{y_1=0} \Omega_{2n}^{\text{loop}} =&  \underbrace{D \, \cdot \prod_i \frac{\diff y_i}{y_i^2} \prod u_C^{X_C} }_{(\star)}\quad + \quad  \prod_i \frac{\diff y_i}{y_i^2} \prod u_C^{X_C}\left[ \underbrace{\sum_{j<k \in \{2,\dots,2n\}} X_{k,j} \left( \frac{\partial \log{u_{j,k}^{S.I.}}}{\partial y_{1}} + \frac{\partial \log{u_{k,j}}}{\partial y_{1}} \right)}_{(\star \star)} \right. \\
	& \left. +  \underbrace{\sum_{j \in \{2,\dots,2n\}} Y_j \frac{\partial \log{u_{Y_j}}}{\partial y_{1}}}_{(\star \star \star)} \quad +\quad  \underbrace{ \sum_{j\in\{3,\dots,2n-1\}}X_{1,j} \left(\frac{\partial \log{u_{j,1}}}{\partial y_{1}} +\frac{\partial \log{u_{1,j}^{S.I.}}}{\partial y_{1}} + \frac{\partial \log{u^{S.I.}_{j,1}}}{\partial y_{1}}\right)}_{(\star \star \star \star)} \quad \right. \\
	& \left. \left. + \underbrace{X_{1,1} \left(\frac{\partial \log{u_{1,1}}}{\partial y_{1}} + \frac{\partial \log{u^{S.I.}_{1,1}}}{\partial y_{1}}\right)}_{(\star \star \star \star \star)} -1 \right]\right\vert _{y_{1,p}=y_{1^\prime,p}=0}.
\end{aligned}
\label{eq:loopcut2}
\end{equation}

Now since $X_{k,j} = X_{j,k}$, from figures \ref{fig:LoopCut} and \ref{fig:TreeGlue}, we can see that these variables correspond to the ones present in $(\dagger \dagger)$ in the tree-level glue side. The only subtlety is that on the loop side, we have $X_{1,2n}=X_{1,2}=0$ and these don't have to be zero on the tree side. However, setting these to zero on the tree side will not introduce any new poles, and therefore for the matching we set them to zero as well. In addition, from figures \ref{fig:LoopCut} and \ref{fig:TreeGlue}, we can also check that $Y_j$ on the loop side maps to $X_{p,j}$ on the tree glue side.  Finally, the choice of triangulation for the loop/tree problems makes it clear that $\prod_i \frac{\diff y_i}{y_i^2} \prod u_C^{X_C}$ is the same for both of them. 
  
The approach we will follow is to analyze each term separately and understand whether they match directly or differ by a total derivative. The matching works quite intricately, and we devote the appendix~\ref{sec:matchingAll} for more details, here we simply summarize the results. 

Both $(\star)$ and $(\star \star)$ can be shown to match $(\dagger)$ and $(\dagger \dagger)$, respectively. The same is not true for the remaining three terms, however, the difference will be shown to be the following rather non-trivial total derivative:
\begin{equation}
    -\frac{\partial}{\partial y_t} \left(\prod \frac{1}{y_i^2} \frac{\prod_{k\in\{1, \dots, m-1\}} u_{p,k}u_{1^\prime,k}}{u_{1,p}\prod_{j\in\{2, \dots, 2n\}} u_{p,j}^2} \prod_{C} u_C^{X_{C}}\right)\bigg \vert_{y_{1,p}=y_{1^\prime,p}=0}.
\end{equation}

It is very pleasing that the total derivative is with respect to the only variable we could possibly have ``local" to the triangulation. 

This establishes the consistency of our curve integral for scalar-scaffolded gluons, by showing that the loop-cut and the tree-level gluing agree up to a total derivative. We stress again that while this argument is strictly valid at 1-loop, its quite ``local" character makes it likely that it can be extended to any number of loops. 

\subsection{Tree-Loop Cut}
\textcolor{red}{Copied from letter.}
\begin{equation}
\begin{aligned}    \mathop{\mathrm{Res}}_{X_{a,b}=0}\left(\Omega_{2n}^{\text{loop}}\right) &= \sum_{j \in L, J\in R} \left[\left(X_{j,J}-X_{j,b}\hat{\delta}_{j,b-1} - X_{a,J}\right) \frac{\partial \mathcal{A}_L^\mathcal{S}}{\partial X_{j,x}}\frac{\partial \mathcal{I}_R^\mathcal{S}}{\partial X_{x^\prime,J}} + \left(X_{J,j}-X_{j,b}\hat{\delta}_{j,b-1}  - X_{J,a}\hat{\delta}_{J,a-1} \right) \frac{\partial \mathcal{A}_L^\mathcal{S}}{\partial X_{j,x}}\frac{\partial \mathcal{I}_R^\mathcal{S}}{\partial X_{J,x^\prime}}\right]\\
&\quad + \sum_{j\in L} \left[\left(X_{j,p} - X_{a,p} -X_{j,b}\hat{\delta}_{j,b-1}\right)   \frac{\partial \mathcal{A}_L^\mathcal{S}}{\partial X_{j,x}}\frac{\partial \mathcal{I}_R^\mathcal{S}}{\partial X_{x^\prime,p}}\right] + \sum_{j\in L} X_{a-1,a} \frac{\partial \mathcal{A}_L^\mathcal{S}}{\partial X_{j,x}}\frac{\partial \mathcal{I}_R^\mathcal{S}}{\partial X_{a-1,a}} \bigg\vert_{x^\prime \rightarrow a},
\end{aligned}  
\label{eq:tree-loop}
\end{equation}
with $\hat{\delta}_{i,k} = 1-\delta_{i,k}$, $L=(a+1,a+2,\cdots,b-1)$, and $R=(b,b+1,\cdots,a-1,a)$. 
